Good SFT Optimizes for SFT, Better SFT Prepares for Reinforcement Learning

Post-training of reasoning LLMs is a holistic process that typically consists of an offline SFT stage followed by an online reinforcement learning (RL) stage. However, SFT is often optimized in isolation to maximize SFT performance alone. We show that, after identical RL training, models initialized from stronger SFT checkpoints can significantly underperform those initialized from weaker ones. We attribute this to a mismatch typical in current SFT-RL pipelines: the distribution that generates the offline SFT data can differ substantially from the policy optimized during online RL, which learns from its own rollouts. We propose PEAR (Policy Evaluation-inspired Algorithm for Offline Learning Loss Re-weighting), an SFT-stage method that corrects this mismatch and better prepares the model for RL. PEAR uses importance sampling to reweight the SFT loss, with three variants operating at the token, block, and sequence levels. It can be used to augment standard SFT objectives and incurs little additional training overhead once probabilities for the offline data are collected. We conduct controlled experiments on verifiable reasoning games and mathematical reasoning tasks on Qwen 2.5 and 3 and DeepSeek-distilled models. PEAR consistently improves post-RL performance over canonical SFT, with pass at 8 gains up to a 14.6 percent on AIME2025. Our results suggest that PEAR is an effective step toward more holistic LLM post-training by designing and evaluating SFT with downstream RL in mind rather than in isolation.

==> algos/1_general.tex <==
% helper macro for stop-gradient / detached weights
% \newcommand{\sg}[1]{\mathop{\mathrm{sg}}\!\left[#1\right]}

% % (optional) helper macro for clipping (purely notational)
% \newcommand{\clip}[3]{\mathrm{clip}\!\left(#1,#2,#3\right)}
% \begin{algorithm}[t]
% \caption{\textsc{\name}: Importance-Weighted Offline Loss (weights-focused)}
% \label{alg:unified_train}
% \footnotesize
% \begin{algorithmic}[1]
% \Require Dataset $\mathcal{D}=\{(x,y,R)\}$ with $y=(y_1,\ldots,y_T)$; model $\pi_\theta$;
% logging policy $\pi_\beta$ (or stored $\log\pi_\beta$); block size $B$; discount $\gamma$;
% token loss $\ell_\theta(x,y_{<t},y_t)$.
% \Require Log-ratio clip bounds $[\ell_\Delta, u_\Delta]$; weight clip bounds $[G_{\min},G_{\max}]$.
% \For{each update step}
%   \State Sample minibatch $\mathcal{B}\subset\mathcal{D}$; \quad $L \gets 0$.
%   \For{each $(x,y,R)\in\mathcal{B}$}
%     \State Partition $\{1,\ldots,T\}$ into $K=\lceil T/B\rceil$ contiguous blocks $\{\mathcal{I}_k\}_{k=1}^K$.
%     \For{$t\gets 1$ \textbf{to} $T$}
%       \State $\log\Delta_t \gets \log\pi_\theta(y_t\mid x,y_{<t})-\log\pi_\beta(y_t\mid x,y_{<t})$.
%       \State $\log\Delta_t \gets \clip{\log\Delta_t}{\ell_\Delta}{u_\Delta}$ \algc{token-level ratio clipping}
%     \EndFor
%     \State $\widehat{\mathbf{G}} \gets \textsc{TokenWeight}\!\left(R,\{\log\Delta_t\}_{t=1}^T,\{\mathcal{I}_k\}_{k=1}^K,\gamma\right)$.
%     \For{$k\gets 1$ \textbf{to} $K$}
%       \State $\widehat{\mathbf{G}}_k \gets \clip{\widehat{\mathbf{G}}_k}{G_{\min}}{G_{\max}}$ \algc{weight clipping}
%       \State $L \gets L + \sg{\widehat{\mathbf{G}}_k}\sum_{t\in\mathcal{I}_k}\ell_\theta(x,y_{<t},y_t)$.
%     \EndFor
%   \EndFor
%   \State Take a gradient step on $\frac{1}{|\mathcal{B}|}L$.
% \EndFor
% \end{algorithmic}
% \end{algorithm}

% \begin{algorithm}[t]
% \caption{\textsc{\name}: Importance-Weighted Offline Loss (block-wise suffix IS)}
% \label{alg:unified_train}
% \footnotesize
% \begin{algorithmic}[1]
% \Require Dataset $\mathcal{D}=\{(x,y,R)\}$ with $y=(y_1,\ldots,y_T)$; model $\pi_\theta$;
% logging policy $\pi_\beta$ (or stored $\log\pi_\beta$);
% block size $B$; discount $\gamma$; token loss $\ell_\theta(x,y_{<t},y_t)$.
% \Require IS-ratio clipping bounds $\Delta_{\min},\Delta_{\max}$ (equiv. $\log\Delta_{\min},\log\Delta_{\max}$);
% weight clipping bounds $G_{\min},G_{\max}$.
% \For{each update step}
%   \State Sample minibatch $\mathcal{B}\subset\mathcal{D}$.
%   \State $L \gets 0$.
%   \For{each $(x,y,R)\in\mathcal{B}$}
%     \State Partition $\{1,\ldots,T\}$ into $K=\lceil T/B\rceil$ contiguous blocks $\{\mathcal{I}_k\}_{k=1}^K$.
%     \Statex \algc{\emph{Step 1: compute (clipped) token-wise log importance ratios under teacher forcing.}}
%     \For{$t\gets 1$ \textbf{to} $T$}
%       \State $\log\Delta_t \gets \log\pi_\theta(y_t\mid x,y_{<t})-\log\pi_\beta(y_t\mid x,y_{<t})$.
%       \State $\log\Delta_t \gets \clip{\log\Delta_t}{\log\Delta_{\min}}{\log\Delta_{\max}}$.
%       {clip ratios to control variance / avoid rare huge weights}
%     \EndFor
%     \Statex \algc{\emph{Step 2: turn terminal feedback into per-block weights via suffix IS.}}
%     \State $\widehat{\mathbf{G}} \gets \textsc{TokenWeight}\!\left(R,\{\log\Delta_t\}_{t=1}^T,\{\mathcal{I}_k\}_{k=1}^K,\gamma, G_{\min},G_{\max}\right)$.
%     \Statex \algc{\emph{Step 3: weighted loss; detach weights so we only optimize the likelihood objective.}}
%     \For{$k\gets 1$ \textbf{to} $K$}
%       \State $L \gets L + \sg{\widehat{\mathbf{G}}_k}\;\sum_{t\in\mathcal{I}_k}\ell_\theta(x,y_{<t},y_t)$.
%       \algc{$\widehat{\mathbf G}_k$ weights the entire block's token losses}
%     \EndFor
%   \EndFor
%   \State Update $\theta$ using $\frac{1}{|\mathcal{B}|}L$.
% \EndFor
% \end{algorithmic}
% \end{algorithm}

% stop-gradient / detached weights



\newcommand{\sg}[1]{\mathop{\mathrm{sg}}\!\left[#1\right]}
\newcommand{\clip}[3]{\mathrm{clip}\!\left(#1,#2,#3\right)}

\begin{algorithm}[t]
\caption{\textsc{\name}: Compute block weights and a weighted offline loss (one minibatch)}
\label{alg:pear_simple_batch}
\footnotesize
\begin{algorithmic}[1]
\Require Minibatch $\mathcal B=\{(x,y)\}$ with $y=(y_1,\ldots,y_T)$; model $\pi_\theta$; logging policy $\pi_\beta$.
\Require Block size $B$; mode $\mathtt{uniform}$ (sequence-level) or $\mathtt{suffix}$ (continuation-based).
\Require Discount $\gamma\in(0,1]$; token loss $\ell_\theta(x,y_{<t},y_t)$.
\Require Log-ratio clip bounds $[\ell_\Delta,u_\Delta]$; optional weight clip bounds $[G_{\min},G_{\max}]$.
\Ensure Weighted minibatch loss $L(\theta)$.

\State $L \gets 0$
\ForAll{$(x,y)\in \mathcal B$}
  \State Partition $\{1,\ldots,T\}$ into $K=\lceil T/B\rceil$ contiguous blocks $\{\mathcal I_k\}_{k=1}^K$;
         $e_k \gets \max \mathcal I_k$.

  \State \textbf{Step 1: token compatibility (log ratios).}
  \For{$t=1$ to $T$}
    \State $\delta_t \gets \log\pi_\theta(y_t\mid x,y_{<t})-\log\pi_\beta(y_t\mid x,y_{<t})$
    \State $\delta_t \gets \clip{\delta_t}{\ell_\Delta}{u_\Delta}$
  \EndFor

  \State \textbf{Step 2: compress to blocks.}
  \For{$k=1$ to $K$}
    \State $\rho_k \gets \sum_{t\in\mathcal I_k}\delta_t$ \Comment{block log-ratio}
  \EndFor
  \State $S \gets \sum_{k=1}^K \rho_k$ \Comment{full-sequence log ratio}

  \State \textbf{Step 3: assign one weight per block and apply it to block loss.}
  \State $u \gets 0$ \Comment{running suffix sum $u=\sum_{m=k+1}^{K}\rho_m$}
  \For{$k=K$ downto $1$}
    \If{$\mathtt{uniform}$} \Comment{same weight for all blocks: $G \equiv w_{1:T}$}
      \State $\log G_k \gets S$
    \Else \Comment{continuation after block $k$}
      \State $\log G_k \gets (T-e_k)\log\gamma + u$
    \EndIf
    \State $G_k \gets \exp(\log G_k)$
    \State $G_k \gets \clip{G_k}{G_{\min}}{G_{\max}}$
    \State $L \gets L + \sg{G_k}\sum_{t\in\mathcal I_k}\ell_\theta(x,y_{<t},y_t)$
    \State $u \gets u + \rho_k$
  \EndFor
\EndFor
\State \Return $L/|\mathcal B|$
\end{algorithmic}
\end{algorithm}


==> algos/2_subroutine.tex <==
% \begin{algorithm}[t]
% \caption{\textsc{TokenWeight}:(sequence-level is $K{=}1$)}
% \label{alg:unified_weights}
% \footnotesize
% \begin{algorithmic}[1]
% \Require Terminal $R$; $\{\log\Delta_t\}_{t=1}^T$; blocks $\{\mathcal{I}_k\}_{k=1}^K$; $\gamma\in(0,1]$.
% \State $S_{\mathrm{tot}}\gets 0$.
% \For{$k=1$ to $K$}
%   \State $\log\Delta^{\mathrm{blk}}_k \gets \sum_{t\in\mathcal{I}_k}\log\Delta_t$.
%   \State $S_{\mathrm{tot}}\gets S_{\mathrm{tot}}+\log\Delta^{\mathrm{blk}}_k$.
% \EndFor
% \If{$K=1$} \Comment{full-sequence IS}
%   \State $\widehat{\mathbf{G}}_1 \gets R\cdot \exp(\log\Delta^{\mathrm{blk}}_1)$.
%   \State \Return $\widehat{\mathbf{G}}$.
% \EndIf
% \State $P \gets 0$. \Comment{prefix sum up to block $k$}
% \For{$k=1$ to $K$}
%   \State $P \gets P+\log\Delta^{\mathrm{blk}}_k$.
%   \State $\log w_{k+1:K} \gets S_{\mathrm{tot}}-P$. \Comment{suffix sum; $\log w_{K+1:K}=0$}
%   \State $\widehat{\mathbf{G}}_k \gets \gamma^{K-k}\,R\cdot \exp(\log w_{k+1:K})$.
% \EndFor
% \State \Return $\widehat{\mathbf{G}}$.
% \end{algorithmic}
% \end{algorithm}
\begin{algorithm}[t]
\caption{\textsc{TokenWeight} (suffix/sequence IS; sequence-level is $K{=}1$)}
\label{alg:unified_weights}
\footnotesize
\begin{algorithmic}[1]
\Require Terminal $R$; token log-ratios $\{\log\Delta_t\}_{t=1}^T$;
blocks $\{\mathcal{I}_k\}_{k=1}^K$; discount $\gamma\in(0,1]$.
\Require Optional suffix-log clip bounds $[\ell_w,u_w]$.
\State \algc{Aggregate token ratios into block ratios}
\For{$k=1$ to $K$}
  \State $\log\Delta^{\mathrm{blk}}_k \gets \sum_{t\in\mathcal{I}_k}\log\Delta_t$.
\EndFor
\If{$K=1$} \algc{full-sequence IS}
  \State $\log w \gets \log\Delta^{\mathrm{blk}}_1$.
  \State $\widehat{\mathbf{G}}_1 \gets R\cdot \exp(\log w)$.
  \State \Return $\widehat{\mathbf{G}}$.
\EndIf

\State \algc{Compute suffix log-weight for each block}
\State $s \gets 0$ \algc{running suffix sum}
\For{$k=K$ to $1$}
  \State $\log w^{\mathrm{suf}}_k \gets s$.
  \State $s \gets s + \log\Delta^{\mathrm{blk}}_k$.
\EndFor

\For{$k=1$ to $K$}
  \State $\log w^{\mathrm{suf}}_k \gets \clip{\log w^{\mathrm{suf}}_k}{\ell_w}{u_w}$ \algc{suffix clipping}
  \State $\widehat{\mathbf{G}}_k \gets \gamma^{K-k}\, R \cdot \exp(\log w^{\mathrm{suf}}_k)$.
\EndFor
\State \Return $\widehat{\mathbf{G}}$.
\end{algorithmic}
\end{algorithm}


==> algos/even_simpler_algo.tex <==
% \newcommand{\sg}[1]{\mathop{\mathrm{sg}}\!\left[#1\right]}
% \newcommand{\clip}[3]{\mathrm{clip}\!\left(#1,#2,#3\right)}
% \newcommand{\StateCont}{\Statex\hspace{\algorithmicindent}}

% \begin{algorithm}[h]
% \caption{\textsc{\name} (intuitive routine)}
% \label{alg:pear_simple_intuitive}
% \footnotesize
% \begin{algorithmic}[1]
% \Require One example $(x,y)$ with $y=(y_1,\ldots,y_T)$; model $\pi_\theta$;
% \StateCont behavior policy $\pi_\beta$.
% \Require Block size $B$; mode $\mathtt{uniform}$ or $\mathtt{suffix}$;
% \StateCont discount $\gamma\in(0,1]$.
% \Require Token loss $\ell_\theta(x,y_{<t},y_t)$; clip bounds $[\ell_\Delta,u_\Delta]$,
% \StateCont $[G_{\min},G_{\max}]$.
% \Ensure Weighted loss $L(\theta)$.

% \State Partition $[T]$ into $K=\lceil T/B\rceil$ contiguous blocks $\{\mathcal I_k\}_{k=1}^K$;
% \StateCont let $e_k=\max\mathcal I_k$ (the block endpoint).

% \State \textbf{Step 1: compute token signals (vectorized).}
% \State $\delta_{1:T} \gets \clip{\log\pi_\theta(y_t\mid x,y_{<t})-\log\pi_\beta(y_t\mid x,y_{<t})}{\ell_\Delta}{u_\Delta}\ \ \text{for }t\in[T]$
% \State $\ell_{1:T} \gets \ell_\theta(x,y_{<t},y_t)\ \ \text{for }t\in[T]$

% \State \textbf{Step 2: reduce to blocks.}
% \State $\rho_k \gets \sum_{t\in\mathcal I_k}\delta_t,\quad b_k \gets \sum_{t\in\mathcal I_k}\ell_t,\quad \forall k\in[K]$
% \StateCont $\rho_k$ is the (clipped) block log-ratio; $b_k$ is the block loss.

% \If{$\mathtt{uniform}$}
%   \State $\widehat{G} \gets \clip{\exp\!\big(\sum_{k=1}^K \rho_k\big)}{G_{\min}}{G_{\max}}$
%   \State \Return $\displaystyle \sum_{k=1}^{K}\sg{\widehat{G}}\; b_k$
%   \StateCont \algc{same weight for all tokens/blocks: ``is the whole trajectory plausible under $\pi_\theta$?''}
% \Else
%   \State \textbf{Step 3: suffix continuation weights (one suffix-cumsum, no explicit scan).}
%   \State $U_k \gets \sum_{m=k+1}^{K}\rho_m\quad \forall k\in[K]$
%   \StateCont \algc{$U_k$ is the log-ratio of the \emph{future continuation} after block $k$ (suffix sum)}
%   \State $\widehat{G}_{e_k} \gets \clip{\exp\!\big((T-e_k)\log\gamma + U_k\big)}{G_{\min}}{G_{\max}}\quad \forall k\in[K]$
%   \State \Return $\displaystyle \sum_{k=1}^{K}\sg{\widehat{G}_{e_k}}\; b_k$
%   \StateCont \algc{each block weighted by how plausible its \emph{remaining suffix} is under $\pi_\theta$}
% \EndIf
% \end{algorithmic}
% \end{algorithm}


==> sections/2_mismatch_backup.tex <==

\section{Offline Performance May Not Entail Online}

\hao{this sec reads below the standard of your past writing. i assume it will be polished and am not leaving detaield comments now. please make sure the phrasing is precise}
\hao{results should be included here}
\begin{figure}
\centering
\includegraphics[width=.9\linewidth]{plot/offline_online_synlogic_combined_id_pass@8.pdf}
    \caption{Offline v.s. Online pass@8 on SynLogic Games.Both sizes exhibit significant ordering changes, indicating offline performance will not entail online performance.\dylan{we will replace this figure for better clarity}
    \hao{suggest using pass@1 here, unless pass@8 is the standard practice}
    \hao{those colors are too close to distinguish}
    \hao{both plots are too tall and narrow. consider moving the legnd to the right of both plots}
    }
    \label{fig:offline_online}
\end{figure}

\begin{takeawaybox}
\begin{itemize}\itemsep0.2em
\item Objectives optimizing offline performance may not improve RL performance.
\item Intuitive characteristics for offline-trained models cannot prescribe the best RL starting point.
\end{itemize}
\end{takeawaybox}
\hao{suggest moving the takeaway towards the end}
Modern post-training for reasoning is rarely a single-stage optimization~\cite{shao2024deepseekmath,Guo_2025,yang2024qwen25}: we first run an offline
fine-tuning stage (typically SFT) on top of pre-trained models to obtain an initial checkpoint $\pi_0$ (e.g., SFT and its variants), and then proceed with an online RL stage to obtain the final model $\pi_{\mathrm{RL}}$.

Consequently, the offline objective should not target immediate offline scores, a better initialization for subsequent on-policy RL.
\hao{some context that existing approach often optimize for sft alone, even the end goal is an rl-ed model.
be careful about the tone - many works don't do rl and we should not assume every model should undergo rl
}
\hao{lay out the key RQ of this sec up front}
\paragraph{Empirical observation: offline gains can vanish or reverse after RL.}
\hao{i'd make this section more self-contained.
introduce the experimental setting, methods, data, briefly; the details can go to the appendices
}
Prior work has shown that even simple modifications to standard NLL can improve offline performance. However, these offline improvements do not reliably translate to the \emph{post-RL} checkpoint. In Figure~\ref{fig:offline_online}, we analyze multiple modifications\hao{what are these modifications? are they prior works? are they what we invented? it would be more credible if they are common things that people try, or come from prior works}
\hao{also, modification is a weird word choice. suggest method/approach/technique}
that improved upon vanilla NLL and show that the relative ordering of objectives can change after on-policy RL, similar to the effect identified by~\citet{kang2025quagmiressftrlposttraininghigh} for SFT training on different datasets.  We defer more details to Sec~\S~\ref{sec:exp_rank_reversal}.

\paragraph{Commonly used descriptors\hao{bad word choice} do not prescribe good RL initialization\hao{i don't like this framing. -> initial policy}.}
\label{sec:goodness_metrics_not_enough}

% Another natural move is to characterize checkpoints using common
% descriptors used to analyze LM characteristics such as KL-to-base, entropy/diversity, or parameter/gradient drift and update sparsity.

% These descriptors are useful for \emph{describing} differences between checkpoints (e.g., how much the
% policy deviates, how stochastic its samples are, or whether it forgets), but our study suggests they
% do not \emph{predict} which checkpoint will benefit most from RL.
% \todo{Discuss the past metrics and why those may / may not work}

% While studies point out certain characteristics are 

Another natural move is to characterize checkpoints with simple diagnostic metrics. 
While intuitively, offline pass@K with large K~\cite{yue2025doesreinforcementlearningreally} and majority voting accuracy~\cite{kang2025quagmiressftrlposttraininghigh} may correlate with the RL performance, we show (in Figure~\ref{fig:offline_metrics}) that the ranking is not always well-preserved when comparing the effectiveness of \textbf{offline training objectives}\hao{wrong word?}. This renders such criteria inaccurate when used as indicators to evaluate offline objective effectiveness in warm-starting RL.


Offline metrics can describe the model’s current behavior on a fixed
evaluation protocol, but hey are not \emph{causal} with respect to downstream RL performance because they do not capture how the
offline objective shapes future behavior under on-policy training, which is the mechanism through which RL improvements arise.

% The rank reversals above suggest that the offline stage must do more than fitting logged data — it must shape the learning signal that the subsequent on-policy phase will act on.


==> sections/game_backup.tex <==
% \section{Experiments}

% To rigorously evaluate the effectiveness of our approach while taking into consideration any potential confounding factors, we perform two sets of experiments: i) on programmatic-ally generated and verifiable reasoning games arcoss model families and sizes, and ii) math reasoning. 

% \subsection{Games}
% We evaluate training and 
% \subsubsection{Setting}

% We use synthetic puzzles from SynLogic and Enigmata. \todo{What puzzles? how did we select these tasks}. 

% \paragraph{Offline Training Data} 

% We generated \todo{number} puzzles in total \todo{details}. 

% We sampled trajectories from \textsc{Qwen3-8B} and verified the final answers for correctness, resulting in a total of roughly 100,000 trajectories from \todo{check num. prob} puzzles. 
% \todo{Deduplication between train and test}

% \paragraph{Baseline Approaches}
% \todo{Include details of baseline approaches}

% \paragraph{Training Details}

% We train \name with $\gamma=0.999$, clip range for $\hat{G_t}$ to be $[-10,5]$ and per-decision $\Delta_t$ clip to be $[-0.08,0.3]$ for numerical stability. We use $lr=3\times10^{-5}$ for logic games and $lr=1\times10^{-5}$ for math. We train all models for 1 epoch. 

% \paragraph{Online Training}
% We applied standard GRPO with learning rate of 1e-6, batch size of 128, KL coefficienct 0.01. 
% \todo{DAPO?}

% \subsubsection{\name Benefits Online RL}
% We compare post-RL performances for models initialized from \name agains those from other offline training objectives. 
% With the same training data, the model RL'ed from \name-trained offline checkpoint leads to better overall performance over standard SFT and other modified offline training objectives \todo{({+ abs}, {+ rel\%} over {best baseline}).}, across various model families, sizes and both reasoning puzzles and math tasks. 


% Additionally, this benefit can be hidden during the offline training stage, as we have discussed in section \todo{Link to previous section} --- only revealed after online RL training. The reward structure we built into the model is not expected to immediately benefiting the task performance out-of-the-box but impacted its downstream RL efficacy.  

% \subsection{Rank reversals after RL.}
%  Figure {X} reports performance (i) immediately after offline training ($\pi_0$) and (ii) after running identical online RL ($\pi_{\mathrm{RL}}$) from each checkpoint. While {objective A} is best offline, it is overtaken by {objective B / \name} after RL .../

% \subsection{ Why common descriptors fail. }
% We analyze standard checkpoint descriptors—{KL-to-base, entropy, gradient drift/sparsity}—and find they are descriptive but not predictive: checkpoints with similar {KL/entropy} can diverge substantially in post-RL gains, and “closer to base” is not consistently better (or worse). This supports the view that what matters is not a static property of the checkpoint, but how it interacts with the subsequent RL update.

 
% \textbf{Why this matters for post-training.} These gains are not merely offline quality improvements: they reflect a better starting point for RL, i.e., a checkpoint that translates a fixed online compute budget into a stronger final policy.





% \subsubsection{Behavior of \name-trained models}
% \todo{discuss individual metrics \& descriptors of training dynamics}
% We demonstrate that, the models trained with our objective demonstrates distinct characteristics in multiple aspects compared with standard SFT. Additionally, various update objectives exhibit distinct features trained on the same offline data. 
% \paragraph{Reasoning Patterns}

% Since offline learning stage aims to prepare language models for online RLVR with inference-time scaling by equipping it with sophisticated reasoning behaviors, it is important that we examine whether these are preserved with \name-training. 

% We \todo{Detail what we did}. In \todo{Figure}, we show that the reasoning pattern distribution did not significantly differ from SFT. This ensures that the reasoning anchors are well-preserved with \name objective, thus could enable effective prolongedand sophisticated thinking during online RL. 

% \paragraph{Sparsity of parameter update}

% \paragraph{}

% \subsubsection{}

% \todo{include results on OOD performance -- argue non-informative, in the appendix}

\section{Experiments}
\label{sec:experiments}
% \begin{takeawaybox}
% \begin{itemize}\itemsep0.2em
%     \item \name boosts \emph{post-RL} performance for both SFT and KD objectives under a fixed GRPO budget.
%     \item 
% \end{itemize}
% \end{takeawaybox}

\subsection{Overview and evaluation protocol}
\label{sec:exp_overview}
\begin{figure}
    \centering
    \includegraphics[width=.98\linewidth]{plot/qwen3_online_perf_unstack_bar_plot_pass@1.pdf}
    \caption{Pass@1 comparison across initializations for SynLogic Games. \namebasic significantly improve upon SFT initialization, and incorprorating negative gradients can further improve Pass@1. }
    \label{fig:synlogic_results_basic}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=.98\linewidth]{plot/qwen3_is_kd_unstack_perf_bar_plot_pass@8_horizontal.pdf}
    \caption{KD.\todo{offline?}
    }
    \label{fig:synlogic_results_basic}
\end{figure}

\todo{revise}
We evaluate \name as an \emph{offline initialization objective} for subsequent online RL on long-horizon reasoning.
Accordingly, every method is assessed under the same two-stage post-training protocol:
(i) \textbf{Offline stage:} train an initialization on a fixed offline buffer using a chosen objective;
(ii) \textbf{Online stage:} starting from $\pi_0$, run identical online RL (same algorithm, reward, and compute budget)
to obtain a post-online RL performance.

% What to include:
% - Explicitly state: "fixed offline data, fixed RL budget, same decoding, same reward, same seeds (or multiple seeds)."
% - Define your primary endpoint metric as post-RL performance under a fixed RL budget.

\subsection{Tasks and data}
\label{sec:exp_tasks_data}
% \todo{Justify why we used logical games}
\subsubsection{Logic games}
\label{sec:exp_games}
\paragraph{Task Sources.}
We use synthetic, verifiable puzzles from SynLogic~\cite{liu2025synlogic} and Enigmata~\cite{chen2025enigmata} as a primary testbed.
Both of them are synthetic reasoning environments that procedurally generate verifiable puzzle instances from diverse environments to allow noise-free data collation, training and evaluation. This allows for a minimally confounded evaluation setting, with reduced exposure to knowledge dependence and contamination.
% What to include:
% - What puzzle types exist (e.g., grid/sequence/constraint satisfaction/etc.)
% - How you selected them (coverage, difficulty filtering, removal of degenerate tasks)
\paragraph{Offline buffer construction.}
We generate $\lvert\mathcal{D}_{\text{games}}\rvert \approx$ \todo{N} trajectories by sampling from \textsc{Qwen3-8B}
and verifying final answers.
The resulting offline buffer contains roughly 100,000 trajectories from \todo{M} unique puzzles.
We de-duplicate prompts across train/test and remove any train instances that overlap with evaluation prompts.
% What to include:
% - Exact N trajectories and M puzzles
% - Train/val/test split procedure
% - Dedup rule (exact match / normalized match) and what fields are deduped

\paragraph{Evaluation.}
We measure Pass@\{1,8\} on a held-out set of puzzles with the original verifiers. \todo{How many puzzles?}

\subsubsection{Math reasoning}
\label{sec:exp_math}
\paragraph{Data.}
For offline training, we use the subset of all math problems in SYNTHETIC-2 dataset~\cite{primeintellect_synthetic2_2025} -- a total of 33,400 unique instructions. We sample responses from Qwen3-8B and verify with final answer, forming a dataset of 100,000 question-response pairs. 

For online RL, we use DAPO-17k dataset~\cite{yu2025dapo}.
% We evaluate on \todo{math dataset name(s)} and construct an offline buffer $\mathcal{D}_{\text{math}}$ of size \todo{N}.
% What to include:
% - The precise dataset(s) and preprocessing
% - Whether verification is automatic (unit tests / symbolic check / string match)
% - Train/test split and contamination controls
\paragraph{Evaluation.}
Following common practice\todo{cite}, we evaluate on MATH-500~\cite{hendrycks2021MATH}, MINERVA~\cite{lewkowycz2022MINERVA}, AIME-2024, AIME-2025~\cite{aime} and AMC-2023.

We report average accuracy across 64 samples to reduce variance and pass@K. 
% \subsection{Offline Objectives Under Consideration}
% \label{sec:exp_methods_compared}
% \begin{itemize}
%     \item \textbf{SFT and KL-regularization:} standard negative log-likelihood (NLL) loss; and KL-regularized nll \(\mathcal{L}(\theta)
% =
% \mathbb{E}_{(x,y)\sim\mathcal{D}}\!\big[-\log \pi_\theta(y\mid x)\big]
% \;+\;
% \beta\,\mathbb{E}_{x\sim\mathcal{D}}\!\left[\mathrm{KL}\!\left(\pi_\theta(\cdot\mid x)\,\|\,\pi_{\rm ref}(\cdot\mid x)\right)\right].\) We alter $\beta \in\{0.03,0.1,0.3,1\}$ for KL-regularized variant.
% \item{\ref}
% \end{itemize}


% \paragraph{SFT Family}
% We compare \name against standard SFT and representative modified offline objectives trained on the same buffer: \\
% \textbf{SFT:} s
% ; \\

% \paragraph{KL-Based Distillation} 
% KL-based distillation objective minimizes token-level KL divergence between their next-token distributions under the same prefix:
% \( \mathcal{L}_{\mathrm{KD}}(\theta)
% =\mathbb{E}_{(x,y)\sim\mathcal{D}}\left[\sum_{t=1}^{T}
% \mathrm{KL}\!\left(\pi_{\beta}(\cdot\mid x,y_{<t})\,\big\|\,\pi_{\theta}(\cdot\mid x,y_{<t})\right)\right].\).

\subsection{Training details}
\label{sec:exp_training_details}

\paragraph{Offline training}
\label{sec:exp_offline_training}
Unless stated otherwise, we train for 1 epoch with learning rate $3\times10^{-5}$ on games and $1\times10^{-5}$ on math.
For \name, we use $\gamma=0.999$, clip $\log\hat{G}_t$ to $[-10,5]$, and clip per-decision $\log\Delta_t$ to $[-0.08,0.3]$.


\paragraph{Online RL}
\label{sec:exp_online_training}
Starting from each offline checkpoint $\pi_0$, we run the same online RL procedure to obtain $\pi_{\mathrm{RL}}$.
We use GRPO~\cite{shao2024deepseekmath} with learning rate $10^{-6}$, batch size 128, and KL coefficient 0.01.

\subsection{Results}
\label{sec:exp_main_results}
\hao{suggest including some learning curve comparisons}
\paragraph{\name improves post-RL performance under a fixed RL budget.}
\label{sec:exp_postrl_gains}
\hao{results w/o rl should also be included}\dylan{I referred back to the figure at the beginning}
Figure~\ref{fig:synlogic_results_basic} demonstrates the gain from initializing model with the basic form of \name over standard SFT across different model sizes. We show a clear margin on both pass@1 and pass@8 across model sizes. Moreover, \name outperforms all previously mentioned techniques in \S~\ref{sec:offline_not_entail_online}. Notably, \name does not outperform these objectives out-of-the-box, and even may not improve upon SFT, since \name is not designed to boost offline scores in isolation, but to better shape the prior for online RL.

We show in Table~\ref{tab:math_results} that \name-initialized model can achieve higher overall performance across common math reasoning benchmarks for multiple model families. 

We also show that \name's weighing scheme can work with KL-based knowledge distillation and further improve upon that by computing the needed quantity using already-computed information. \todo{KD results}

This underscores \name’s generality as a plug-in reweighting module and supports our central diagnosis: offline training should build RL readiness via outcome-aware credit assignment, which is largely absent from likelihood-style objectives.

\paragraph{You need to weigh the future, not a single action.}

Concurrent works proposed several action-level stablizations to SFT, 
\(
\mathcal{L}(\theta)
\;=\;
\mathbb{E}_{(x,y,R)\sim\mathcal{D}}
\left[
\sum_{t=1}^{T} w(x,y_{<t},y_t)\ell_\theta(x,y_{<t},y_t)
\right],\).

% Table~\todo{1} reports post-RL performance when initialized from different offline objectives.
% With identical offline data and an identical online RL set-up, initializing from \name yields stronger final models
% across \todo{model families/sizes} on both logic games and maths.
% Compared to the best baseline, \name improves post-RL performance by \todo{+X abs} (\todo{+Y\% rel}). 


% What to include (write it once, then point to tables):
% - "fixed RL budget" emphasized again
% - "across families/sizes" emphasized with a compact table
% - one sentence explaining practical significance


% \paragraph{Offline performance may not entail online performance}
% \label{sec:exp_rank_reversal}
%  \todo{Fix}

% \begin{figure}
%     \centering
%     \includegraphics[width=.8\linewidth]{plot/offline_online_grad_rotation_qwen3-1.7b-base.pdf}
%     \caption{Mean principal angle between offline and online GRPO gradients starting from the tuned model.}
%     \label{fig:roration angle}
% \end{figure}


% \paragraph{Common checkpoint descriptors are descriptive but not predictive}
% \label{sec:exp_descriptors_fail}
% We analyze standard descriptors of $\pi_0$---\todo{KL-to-base, entropy, parameter drift, update sparsity}---and find
% they do not reliably predict post-RL gains.
% Checkpoints with similar \todo{KL/entropy} can differ substantially in RL improvement, and “closer to base” is not
% consistently better or worse.
% This supports the view that the key property is not a static descriptor of $\pi_0$, but how it interacts with the
% subsequent RL updates.





\begin{figure*}
\centering
  \begin{subfigure}[t]{0.24\linewidth}
    \centering
    \includegraphics[width=\linewidth]{plot/qwen3-1.7b-base_forward_kl_id_pass@8.pdf}
    \caption{Post-RL performance versus offline KL drift.}
    \label{fig:kl}
  \end{subfigure}
  \hfill
  \begin{subfigure}[t]{0.24\linewidth}
    \centering
    \includegraphics[width=\linewidth]{plot/qwen3-1.7b-base_hard_sparsity_id_pass@8.pdf}
    \caption{Post-RL performance versus offline update sparsity.}
    \label{fig:sparsity}
  \end{subfigure}
  \hfill
  \begin{subfigure}[t]{0.24\linewidth}
    \centering
    \includegraphics[width=\linewidth]{plot/qwen3-1.7b-base_avg_nss_id_pass@8.pdf}
    \caption{Post-RL performance versus offline NSS.}
    \label{fig:offline_nss}
  \end{subfigure}
  \begin{subfigure}[t]{0.24\linewidth}
    \centering
    \includegraphics[width=\linewidth]{plot/qwen3-1.7b-base_avg_offline_online_nss_id_pass@8.pdf}
    \caption{Post-RL performance versus online NSS.}
    \label{fig:online_nss}
  \end{subfigure}
    \caption{Stability of offline update}
    \label{fig:model_characteristics}
\end{figure*}
\todo{Depending on space, may trim and move this paragraph to appendix. }


% \begin{figure}
%     \centering
%     \includegraphics[width=.8\linewidth]{}
%     \caption{Rotation of principle angle during GRPO.}
%     \label{fig:roration angle}

%     \label{fig:pipeline}
% \end{figure}
\subsection{\name Transfers to different RL task distributions.}
\label{sec:transfer}

We next test whether the capability induced by \name during offline training transfers to online RL on a
different task distribution. Concretely, we initialize RL from the \name checkpoint and run online training
on the Enigmata training split (\todo{how many trajectories / tasks}), then evaluate on a held-out set of
Enigmata tasks after removing any near-duplicates across splits (\todo{describe dedup: exact-match on
canonicalized prompts, plus fuzzy threshold / hash-based filtering}). As shown in
Table~\ref{tab:synlogic_enigmata}, despite the difference between the offline training domain and the
online RL domain, \name consistently provides a stronger warm start than standard SFT: it achieves better post-RL performance under the same RL recipe and rollout budget.
These results suggest that \name can learn a generalizable RL-useful inductive bias that transfers the OPE-based weighting scheme. 

\subsection{Incorporating Negative Examples}
\label{sec:negative_grad}
We present a variant of \name that stabilizes the offline update negative examples $\mathcal{D}^-=\{(x,y,R)\in\mathcal{D}:R\le 0\}$
via a simple \emph{sequence-level} IS weight with a negative sign. Concretely, we compute \todo{confirm}
\(
W_{1:T}(\tau)\triangleq \prod_{j=1}^{T}\frac{\pi_\theta(a_j\mid s_j)}{\pi_\beta(a_j\mid s_j)},
\)
stabilize it to $\widehat{W}_{1:T}$, and add the auxiliary term
\(
\mathbb{E}_{\tau\sim\mathcal{D}^-}\Big[\sum_{t=1}^{T} \big(-\lambda\,\mathrm{sg}[\widehat{W}_{1:T}(\tau)]\big)\,\ell_\theta(s_t,a_t)\Big]
\)
to the positive-only objective in Eq.~\eqref{eq:iw_sft_main}. This update ``pushes down'' the likelihood of entire
negative sequences while avoiding token-/suffix-level signed ratio products that can be particularly unstable on long horizons. We sub-sampled 50K positive data and included 50K negative data from the same behavior policy on the same set of inistructions. 
\input{tables/math}
From \todo{Figure handle}, we show that under the same data budget, mixing negative trajectories for stabilization can bring significant additional gains to RL over positive-only \name initialization significantly.



\begin{figure}
\centering
  \begin{subfigure}[t]{0.49\linewidth}
    \centering
    \includegraphics[width=\linewidth]{plot/weight_bins_kl_ridge_qwen3-1.7b-base_smooth.pdf}
    \caption{Qwen3-1.7B-Base}
    \label{fig:kl_1_7b}
  \end{subfigure}
  \begin{subfigure}[t]{0.49\linewidth}
    \centering
    \includegraphics[width=\linewidth]{plot/weight_bins_kl_ridge_qwen3-4b-base_smooth.pdf}
    \caption{Qwen3-4B-Base}
    \label{fig:kl_4b}
  \end{subfigure}
    \caption{\name-to-base KL divergence across weight levels. Token distribution is more heavily driven on important tokens that drives success probability. }
    \label{fig:kl}
\end{figure}

==> sections/intro_backup.tex <==
\section{Introduction}
\hao{throughout the paper, we are blurring the boundary between sft and rl and used a lot of 
rl terminologies to describe sft. 
this is fine, but make sure we have introduced enough context since this is not a RL paper 
and the rl jargon will make it less accessible to general llm audience.
i suggest using section 2 to serve a dual purpose of also laying out these terminologies,
on top of its current role.
}
Reasoning post-training is typically two-stage: an \emph{offline} fine-tuning phase produces an initial checkpoint, and an
\emph{online} RL phase further enhance it into the deployed model~\cite{shao2024deepseekmath,Guo_2025,yang2024qwen25}. Both stages have become
active research fronts. On the online side, RL recipes continue to evolve; on the offline side, a growing set of objectives
reweight or regularize next-token likelihood~\cite{qin2025iwsft,zhu2025proximalsft,wu2025dft,lin2025sftdoesnthurtgeneral,li2025beyond} and often improve \emph{offline} scores.

\dylanmodify{However, while existing recipes usually optimize for SFT performance in isolation with the implicit assumption that this will translates to the final performance after online RL stage, we highlight that \textbf{offline performance is an unreliable proxy
for post-RL performance}. Across model families and scales, the apparent ranking of offline objectives can
shrink, disappear, or even reverse after running the \emph{same} RL recipe from each initialization~\cite{kang2025quagmiressftrlposttraininghigh}. Consequently, optimizing offline metrics alone can be a
systematically misleading target when the goal is final post-RL accuracy. Indeed, RLVR’s effectiveness can depend sharply on the initial loss/representation geometry~\citep{zhu2025pathnottaken}.}

% However, the offline checkpoint is not what we ship. It is an initialization for a fixed downstream online RL
% procedure. Therefore, the question is not which offline
% objective looks best in isolation, but which one yields the strongest \emph{post-RL} model under a fixed RL recipe.
\hao{it needs to be more clear that existing recipes often optimizes for sft performance in isolation with the implicit assumption that
it translates to better final perfomance after rl}

% In this work we document a simple but consequential fact: \emph{offline performance is an unreliable proxy
% for post-RL performance}. Across model families and scales, the apparent ranking of offline objectives can
% shrink, disappear, or even reverse after running the \emph{same} RL recipe from each initialization~\cite{kang2025quagmiressftrlposttraininghigh}. Consequently, optimizing offline metrics alone can be a
% systematically misleading target when the goal is final post-RL accuracy. Indeed, RLVR’s effectiveness can depend sharply on the initial loss/representation geometry~\citep{zhu2025pathnottaken}.

% \delete{A natural reaction is to look for stronger offline diagnostics. Recent analyses contrast RL updates with SFT—e.g., changes in KL-to-base, entropy/diversity, or representational movement—and argue that these correlate with desirable behaviors such as reduced forgetting or more targeted updates.~\cite{shenfeld2025rlrazor,zhu2025pathnottaken,chen2025retaining}.} 

% \delete{However, such signatures are largely descriptive: they do not directly quantify how much additional improvement a fixed downstream RL phase can extract from a given initialization, and empirically they do not reliably predict post-RL gains~\todo{cite: stability/forgetting/representation-drift studies in post-training}. We show that matching RL’s diagnostics is not the same as producing an initialization from which downstream RL can consistently improve.}

Our premise is that the offline stage should instead optimize \emph{Online RL readiness}: it should shape the initialization so that, when downstream RL receives sparse terminal feedback, that signal can be attributed to the earlier tokens that made success more likely~\cite{arjonamedina2019rudderreturndecompositiondelayed}. Concretely, RL readiness requires long-horizon, policy-dependent credit assignment—differentiating early decisions by their effect on the probability of eventual success, rather than treating all tokens as equally supervised targets.
\begin{figure*}
\centering
\includegraphics[width=\linewidth]{plot/offline_online_synlogic_combined_1_by_4.pdf}
    \caption{Offline v.s. Online pass@1 on SynLogic Games. It exhibits significant ranking changes indicating offline performance will not entail online performance.
    }
    \label{fig:offline_online}
\end{figure*}
Yet standard SFT and many stabilized or reweighted likelihood variants remain fundamentally behavior-cloning-like: they maximize next-token likelihood under logged prefixes, providing local supervision but does not propagate terminal correctness back through the sequence~\cite{ross2011imitation,mehta2024stablebccontrollingcovariateshift,liu2019offpolicypolicygradientstate,ross2014reinforcementimitationlearninginteractive,sun2017deeplyaggrevateddifferentiableimitation}. As a result, they do not distinguish outcome-critical parts from those unsuccessful in-context search attempts.This mis-aligns offline training with the subsequent online RL phase which optimizes end-of-trajectory success.

% Meanwhile, a growing line of work imports offline RL ideas into LLM post-training from fixed datasets~\cite{lanchantin2025bridgingofflineonlinereinforcement,wang2024oreo,snell2023offlinerlnaturallanguage,baheti2024leftoverlunchadvantagebasedoffline,richemond2024offlineregularisedreinforcementlearning,mukherjee2025offlinerlrewardweightedfinetuning}, arguing that one can directly optimize reward-improving policies from a static buffer of logged generations for language models. We adopt similar lens and treat responses as logged decision trajectories generated by a known behavior
% policy, with reward observed only at the end, but ask a complementary question: how should the
% \emph{offline} update be designed to maximize gains from a \emph{fixed} \emph{online} RL recipe~\cite{xie2022policyfinetuing,huang2023nonadaptive}?
We adopt an offline RL view and treat responses as logged decision trajectories~\cite{lanchantin2025bridgingofflineonlinereinforcement,wang2024oreo,snell2023offlinerlnaturallanguage,baheti2024leftoverlunchadvantagebasedoffline,richemond2024offlineregularisedreinforcementlearning,mukherjee2025offlinerlrewardweightedfinetuning}, and try to address this offline-to-online RL problem~\cite{xie2022policyfinetuing,huang2023nonadaptive}.
\hao{intro up to here should be tigenthed especially the part reviewing prior works}


Inspired by classic off-policy evaluation~\cite{pdis2000,thomas2016dataefficientoffpolicypolicyevaluation,jiang2016doublyrobustoffpolicyvalue,levine2020offlinereinforcementlearningtutorial}, we propose \name (\fullname), a simple \emph{weighting framework} for offline post-training stage that 
\dylanmodify{propagates sparse terminal feedback back to earlier tokens in logged trajectories collected under the behavior policy, so offline learning upweights prefix decisions that make eventual success more likely under the current policy, thereby warm-starting downstream RL with a more outcome-aware initialization.
}
%assigns long-horizon credit to early tokens using terminal feedback, to better warm-start the model for online RL. 
\hao{ it doesn't connect how off-policy eval addresses the problem we laid out earlier}

\name assigns each action a weight by estimating, from the logged continuation, the expected
terminal reward under the current policy’s distribution. Concretely, we apply a per-decision OPE
change-of-measure on the \emph{suffix}: an action at position $t$ is weighted by the terminal reward times an importance
ratio over the logged suffix $t{+}1{:}T$, down-weighting credit when the observed continuation is off-policy for
$\pi_\theta$. Crucially, this weighting is computed without any auxiliary learned modules (e.g., critic/PRM) and only adds minimal total overhead to the standard offline training process.

We evaluate \name against various baselines on both reasoning games and math benchmarks across \todo{model families and scales}, followed by a fixed online RL recipe. \name and its multiple variants consistently improves \emph{post-RL} performance over strong offline baselines,  We show that \name is compatible with both NLL loss and reverse-KL based KD objectives, yielding up to
\todo{$x$} absolute gains (\todo{metric: pass@k / accuracy}) for \todo{Benchmarks}. We demonstrate that \name does the heavy-lifting for model update during offline stage, allowing the online RL stage to achieve the best performance with milder drifts from offline locality. 



==> sections/method_backup.tex <==
\section{Method}
\label{sec:method}

To reliably improve post-RL performance, we seek to design an \emph{offline} objective that produces a stronger initialization for subsequent \emph{online}
RL on reasoning tasks. We assume logged responses with terminal
feedback and want the offline update to reflect how early decisions affect downstream correctness.
Throughout, we view generation as a sequential decision process and derive token-level (and optionally
\emph{block-wise}) credit weights from terminal feedback.

\paragraph{Why uniform SFT is misaligned.}
\hao{this one fits better in section 2. 
}
Standard supervised fine-tuning (SFT) uniformly maximizes next-token likelihood under the logged
prefix distribution. Like behavior cloning in RL, this is a one-step objective of matching the logged next token given a logged prefix without accounting for how that decision influences future ones and ultimately the terminal success. When the learned policy deviates from the logging policy, this induces covariate shift in the visited prefix distribution; errors made under these off-logged prefixes are not corrected by the training signal and therefore compound over long horizons~\cite{ross2011imitation,mehta2024stablebccontrollingcovariateshift,liu2019offpolicypolicygradientstate,ross2014reinforcementimitationlearninginteractive,sun2017deeplyaggrevateddifferentiableimitation}.

In long-form (R1-style~\cite{Guo_2025}) reasoning, a solution trace often invovles search (trial, backtrack, self-correction) etc.
Therefore, logged trajectories typically interleave a small number of \emph{outcome-critical} decisions with many tokens unsuccessful or abandoned exploration. Applying uniform supervision on each token without distinguishing their effects will make the model imitate exploration artifacts as strongly as decisive choices, leading to snowballing errors during inference.~\cite{kumar2022preferofflinereinforcementlearning,zhou2022real,park2025saliencyawarequantizedimitationlearning}.
\hao{i'm not entirely convinced.
this seems justification for token-level score (credit assignment) or dense reward,
rather than using IS to correct for off-policyness
}

% imitation not only will waste capacity on those artifacts of reasoning, but also 





% Thus early deviations irreversibly change the reachable continuation states~\cite{arora2023exposurebiasmattersimitation}
% and local errors can ``snowball''~\cite{gan2025rethinkingexternalslowthinkingsnowball}. 

% Moreover,
% correctness typically depends on a small subset of tokens (the \emph{correct path}). Horizon-wide
% imitation that also matches erroneous detours wastes capacity and can actively reinforce failure modes,
% leading to suboptimal results.

\paragraph{Key idea.}
% Policy-gradient fine-tuning changes token log-probabilities in proportion to a long-horizon credit
% signal, while SFT and reverse-KL based distillation applies uniform token weights. 
In \name, we construct an \emph{offline} credit weight
from terminal feedback by comparing the target policy to the data-generator along the \emph{logged suffix}.
This yields an importance weight that attributes downstream outcomes back to
earlier decisions. We instantiate this idea using per-decision importance sampling (PDIS) off-policy
evaluation (OPE) inspired by~\citet{pdis2000}. We consider both (i) \emph{token-level} decisions
and (ii) a \emph{block-wise} decisions where $B$ tokens are treated as one macro-action (e.g.,
$B{=}4$ or $B{=}8$), which can reduce effective horizon and stabilize credit assignment.

\begin{figure*}
\centering
\includegraphics[width=.9\linewidth]{figures/pipeline.pdf}
    \caption{Pipeline of \name. We compute the expected value $\hat{G_t}$ of a token $y_t$ by applying change-of-measure following standard OPE with a suffix weight. Then we weigh the gradient of that token with the value.\todo{better description.}}
    \label{fig:offline_online_17b}

    \label{fig:pipeline}
\end{figure*}

\hao{again, i think the math in this sec is overly complicated.
if we plan to sell this as an sft algo, i do not see the point of describing it as a rl algo.
besides, using these rl terminologies will confuse the readers about whether this is the sft stage or the rl stage.
definitely avoid the action/state/reward terminologies, super confusing
}
\hao{suggest an alternative - 
make the description of algo  easy and non technical and avoid using rl terms;
towards the end, write a dedicated discussion (maybe some formal propositions/statements, and even a table saying XX in our algo corresponds to YY in OPE)
to connect it to OPE
}
\subsection{Setup and notation}
\label{sec:setup_iw_sft}

We assume an offline dataset of logged generations with terminal feedback
\[
\mathcal{D}=\{(x^{(n)},y^{(n)},R^{(n)})\}_{n=1}^{N},
\]
where $x$ is a prompt, $y=(y_1,\ldots,y_T)\sim \pi_{\beta}$ is a response from a behavior (or logging) policy distribution, and $R\in\mathbb{R}$ is scalar feedback observed
\emph{at the end of the response}. For readability we write one sample $(x,y,R)\sim\mathcal{D}$. We train a target policy
$\pi_\theta$. In this work, our main focus is verifiable reasoning, where $R\in\{-1,1\}$ indicates whether a verifier determines the final answer to be correct.

For simplicity of notations, we denote the
token-level state/action as
\(
s_t \triangleq (x,y_{<t}),
a_t \triangleq y_t, t=1,\ldots,T,
\)
and view a response as a trajectory $\tau=(s_1,a_1,\ldots,s_T,a_T)$ with terminal reward $R(\tau)\equiv R(x,y)$.

\paragraph{Block-wise decisions (macro-actions) for stability.} \todo{Motivation}
We also support a macro-action variant where $B$ consecutive tokens are treated as one decision (e.g.,
$B\in\{4,8\}$). This reduces the effective horizon to $K=\lceil T/B\rceil$ and can stabilize credit assignment. In this case, denoting the $k$-th block as $A_k$, state before it as $S_k$, we have
$\pi_\theta(A_k \mid S_k) \triangleq \prod_{j\in \mathcal{I}_k}\pi_\theta(a_j\mid s_j)$ where $\mathcal{I}_k$ is the set of indices in $A_k$.
We present the full
formalization in Appendix~\ref{app:blockwise}.
\hao{this should go towards the end. unless this is a very important variant, no need to talk about it twice}



%; in the main text, it suffices to view block-wise training as applying a \emph{piecewise-constant} weight to all tokens inside each block.

\subsection{Credit from terminal feedback via suffix ratios}
\label{sec:q_suffix_is_clean}

Our goal is to turn terminal feedback into \emph{policy-aware, position-dependent} credit weights for the
offline likelihood objective.

\paragraph{Suffix importance ratio.}
Given a logged trajectory $\tau$, define the suffix ratio from $t{+}1$ to $T$:
\begin{equation}
w_{t+1:T}(\tau)
\;\triangleq\;
\prod_{j=t+1}^{T}
\frac{\pi_\theta(a_j\mid s_j)}{\pi_\beta(a_j\mid s_j)} \triangleq \prod_{j=t+1}^{T}\Delta_j .
\label{eq:suffix_w_clean_main}
\end{equation}
$w_{t+1:T}(\tau)$ measures how plausible the \emph{observed continuation} is under the current policy $\pi_{\theta}$
relative to the logging policy $\pi_{\beta}$. Intuitively, when assigning credit to decision $a_t$, we treat the
future $a_{t+1:T}$ as a \emph{reward-to-go carrier}.
%; if the logged continuation is off-distribution for
% $\pi_\theta$, it should contribute less to updating $\pi_\theta$. 
Concretely, credit assigned to $a_t$ via $R(\tau)$ is suppressed when the remainder $a_{t+1:T}$ is relatively implausible under $\pi_\theta$ (small $w_{t+1:T}(\tau)$), and emphasized
only when the logged suffix is approximately reproducible by $\pi_\theta$ (large $w_{t+1:T}(\tau)$).


\paragraph{Per-token credit weight.}
We define the per-token credit weight on the logged trajectory as
\begin{equation}
G_t(\tau)
\;\triangleq\;
\gamma^{\,T-t}\,R(\tau)\,w_{t+1:T}(\tau),
\label{eq:G_def_main}
\end{equation}
where $\gamma\in(0,1]$ is a discount factor used to control how aggressively terminal
feedback is propagated backward in position and acts as variance control in long responses.

Equation~\eqref{eq:G_def_main} is a logged-trajectory instantiation of a per-decision IS rewrite: it
converts a continuation expectation under $\pi_\theta$ into an expectation over logged continuations
from $\pi_\beta$, while holding the logged prefix fixed. \todo{More details in Appendix~\ref{app:pdis}.}    



% The suffix importance ratio $w_{t+1:T}(\tau)$ re-weights each token update by the
% \emph{relative likelihood} of the logged continuation under the current policy $\pi_\theta$ versus the
% behavior policy $\pi_\beta$. Concretely, credit assigned to $a_t$ via $R(\tau)$ is suppressed when the
% remainder $a_{t+1:T}$ is relatively implausible under $\pi_\theta$ (small $w_{t+1:T}(\tau)$), and emphasized
% only when the logged suffix is approximately reproducible by $\pi_\theta$ (large $w_{t+1:T}(\tau)$).
\paragraph{Stabilization.}
In practice, products of ratios can be heavy-tailed. We compute suffix ratios in log-space and apply clipping for each individual weight ratio $\Delta_j$ in the product and the final $w_{t+1:T}$ to ensure stability. 
We denote the stabilized return as $\hat{G_t}(\tau)$. 
More details are in Appendix~\ref{app:stabilizers}.

\subsection{Importance-weighted offline objective}
\label{sec:iw_sft_clean}

Let $\ell_\theta(s_t,a_t)$ denote the loss function applied to each token. For standard SFT, $\ell{_{\theta}^{\text{SFT}}}(s_t,a_t)\triangleq -\log \pi_\theta(a_t\mid s_t)$, for KL-based knowledge distillation, $\ell{_{\theta}^{\text{KD}}}(s_t,a_t)\triangleq \mathrm{KL}[\pi_{\beta}(.|s_t) || \pi_{\theta}(.|s_t)]$

% Let $\ell_\theta(s_t,a_t)\triangleq -\log \pi_\theta(a_t\mid s_t)$ be the token NLL.
% Standard SFT minimizes $\mathbb{E}_{\tau\sim\mathcal{D}}\big[\sum_t \ell_\theta(s_t,a_t)\big]$.

\paragraph{\name}
We replace uniform token loss with the credit-weighted loss from Eq.~\eqref{eq:G_def_main}:
\begin{equation}
{\mathcal{L}_\text{\name}}
\;=\;
\mathbb{E}_{\tau\sim\mathcal{D}}
\left[
\sum_{t=1}^{T}
\mathrm{sg}\!\big[\widehat{G}_t(\tau)\big]\;
\ell_\theta(s_t,a_t)
\right],
\label{eq:iw_sft_main}
\end{equation}
where $\widehat{G}_t$ denotes the \emph{stabilized} version of $G_t$ mentioned above
and $\mathrm{sg}[\cdot]$ is stop-gradient. 

%Note that we do not compute gradients through weights as we use $\widehat{G}_t$ to shape
%credit assignment, not as an auxiliary pathway for %reducing the loss by manipulating the weights.

\paragraph{Practical instantiation.}
We implement
Eq.~\eqref{eq:iw_sft_main} by filtering to the successful subset
$\mathcal{D}^{+}\triangleq\{(x,y,R)\in\mathcal{D}: R=1\}$, which  and avoids instability
that can arise when computing long-horizon ratio products and their stabilizers on failed trajectories. We discuss a variant that incorporates negative trajectories in\S~\ref{sec:negative_grad}.

\paragraph{Block-wise \name.}

We compute one credit weight per block \(\widehat G_k^{\mathrm{blk}}(\tau)\)using the same idea, and apply it uniformly to all tokens inside the block (i.e., piecewise-constant token weights):
\(\mathcal{L}_{\name}^{\mathrm{blk}} =
\mathbb{E}_{\tau\sim\mathcal{D}}\left[
\sum_{k=1}^{K}\mathrm{sg}\!\big[\widehat G_k^{\mathrm{blk}}(\tau)\big]\;
\sum_{t\in\mathcal{I}_k} \ell_\theta(s_t,a_t)
\right].\)
. This trades fine-grained attribution for substantially more stable credit assignment.
\hao{suggest including pseudo code to put everything together}
\hao{close with some discussion on overead/efficiency,
and what to do when there is no access to the behavior policy
}

% The block-wise variant is identical in spirit: we compute one weight per block and apply it to the block
% loss (equivalently, a piecewise-constant token weight within the block). We provide the full definition
% and its equivalence to token weighting in Appendix~\ref{app:blockwise}.

==> tables/math-backup.tex <==
\begin{table*}[t]
\small
\centering
\renewcommand{\arraystretch}{1.05}

% Inline cell for \name: main score + small gain over SFT (pp) at lower-right
\newcommand{\namecell}[2]{%
  {\color{pearfg}#1\%}\hspace{0.15em}%
  \raisebox{-0.15ex}{\smash{\scriptsize\color{orange}(#2)}}%
}

\begin{tabular}{cc|cP cP cP cP}
\hline
\multicolumn{2}{c|}{\textbf{Base Model}} &
\multicolumn{2}{c}{\textbf{Qwen2.5-1.5B-Math}} &
\multicolumn{2}{c}{\textbf{DS-Qwen-1.5B}} &
\multicolumn{2}{c}{\textbf{Qwen3-4B-Base}} &
\multicolumn{2}{c}{\textbf{Qwen3-8B-Base}} \\
\hline
\textsc{Benchmark} & \textsc{Pass@} &
\shortstack{\textsc{SFT}\\[-0.2ex]{\scriptsize\textsc{+GRPO}}} & \shortstack{{\color{pearfg}\textsc{\namebasic}}\\[-0.2ex]{\scriptsize\color{pearfg}\textsc{+GRPO}}} &
\shortstack{\textsc{SFT}\\[-0.2ex]{\scriptsize\textsc{+GRPO}}} & \shortstack{{\color{pearfg}\textsc{\namebasic}}\\[-0.2ex]{\scriptsize\color{pearfg}\textsc{+GRPO}}} &
\shortstack{\textsc{SFT}\\[-0.2ex]{\scriptsize\textsc{+GRPO}}} & \shortstack{{\color{pearfg}\textsc{\namebasic}}\\[-0.2ex]{\scriptsize\color{pearfg}\textsc{+GRPO}}} &
\shortstack{\textsc{SFT}\\[-0.2ex]{\scriptsize\textsc{+GRPO}}} & \shortstack{{\color{pearfg}\textsc{\namebasic}}\\[-0.2ex]{\scriptsize\color{pearfg}\textsc{+GRPO}}} \\
\hline

\multirow{3}{*}{\textbf{AIME24}} & \Pass{1}  &
5\%  & \namecell{8}{+3}  &
1\%  & \namecell{14}{+13} &
13\% & \namecell{15}{+2}  &
15\% & \namecell{19}{+4} \\
& \Pass{8}  &
19\% & \namecell{23}{+4} &
2\%  & \namecell{38}{+36} &
25\% & \namecell{40}{+15} &
35\% & \namecell{41}{+6} \\
& \Pass{64} &
37\% & \namecell{47}{+10} &
7\%  & \namecell{57}{+50} &
43\% & \namecell{60}{+17} &
60\% & \namecell{67}{+7} \\
\hdashline

\multirow{3}{*}{\textbf{AIME25}} & \Pass{1}  &
3\%  & \namecell{8}{+5}  &
1\%  & \namecell{14}{+13} &
7\%  & \namecell{15}{+8}  &
17\% & \namecell{18}{+1} \\
& \Pass{8}  &
14\% & \namecell{24}{+10} &
5\%  & \namecell{35}{+30} &
21\% & \namecell{35}{+14} &
35\% & \namecell{35}{0} \\
& \Pass{64} &
30\% & \namecell{40}{+10} &
17\% & \namecell{53}{+36} &
40\% & \namecell{57}{+17} &
53\% & \namecell{53}{0} \\
\hdashline

\multirow{3}{*}{\textbf{AMC23}} & \Pass{1}  &
42\% & \namecell{47}{+5}  &
20\% & \namecell{56}{+36} &
54\% & \namecell{59}{+5}  &
45\% & \namecell{55}{+10} \\
& \Pass{8}  &
80\% & \namecell{78}{-2}  &
50\% & \namecell{91}{+41} &
83\% & \namecell{88}{+5}  &
75\% & \namecell{85}{+10} \\
& \Pass{64} &
98\% & \namecell{98}{0} &
63\% & \namecell{98}{+35} &
93\% & \namecell{95}{+2}  &
95\% & \namecell{98}{+3} \\
\hdashline

\multirow{2}{*}{\textbf{Olympiad}} & \Pass{1} &
29\% & \namecell{34}{+5}  &
13\% & \namecell{41}{+28} &
41\% & \namecell{46}{+5}  &
32\% & \namecell{40}{+8} \\
& \Pass{8} &
55\% & \namecell{57}{+2}  &
34\% & \namecell{66}{+32} &
60\% & \namecell{66}{+6}  &
60\% & \namecell{65}{+5} \\
\hdashline

\multirow{2}{*}{\textbf{MATH500}} & \Pass{1} &
63\% & \namecell{70}{+7}  &
36\% & \namecell{72}{+36} &
78\% & \namecell{80}{+2}  &
66\% & \namecell{74}{+8} \\
& \Pass{8} &
89\% & \namecell{91}{+2}  &
68\% & \namecell{94}{+26} &
93\% & \namecell{93}{0}  &
90\% & \namecell{93}{+3} \\
\hline

\multicolumn{2}{c|}{\textbf{Pass@1 Avg.}} &
28\% & \namecell{33}{+5} &
14\% & \namecell{39}{+25} &
39\% & \namecell{43}{+4} &
35\% & \namecell{41}{+6} \\
\multicolumn{2}{c|}{\textbf{Pass@8 Avg.}} &
51\% & \namecell{55}{+4} &
32\% & \namecell{65}{+33} &
56\% & \namecell{65}{+9} &
59\% & \namecell{64}{+5} \\
\hline
\end{tabular}

\caption{Post-RL math results with models initialized by standard SFT v.s. vanilla \name-weighted NLL. For stability, \textsc{Pass@1} in AIME24 and AIME25 are averaged over 64 samples.
\hao{the table is very confusing andreaders might think these are sft results}
\hao{it is concerning that we didn't compare to any baseline beyond sft}
\hao{it is perhaps more clear to present these using bar plots similar to figure 2, showing improvements after sft and rl}
}
\label{tab:math_results}
\end{table*}
% \footnotetext{Small numbers next to \name are absolute gains over SFT (percentage points). On averaged rows (left$\rightarrow$right base models), Pass@1 gains are +5/+25/+4/+6 and Pass@8 gains are +4/+33/+9/+5.}

